LOSTIN: Logic Optimization via Spatio-Temporal Information with Hybrid Graph Models

Despite the stride made by machine learning (ML) based performance modeling, two major concerns that may impede production-ready ML applications in EDA are stringent accuracy requirements and generalization capability. To this end, we propose hybrid graph neural network (GNN) based approaches towards highly accurate quality-of-result (QoR) estimations with great generalization capability, specifically targeting logic synthesis optimization. The key idea is to simultaneously leverage spatio-temporal information from hardware designs and logic synthesis flows to forecast performance (i.e., delay/area) of various synthesis flows on different designs. The structural characteristics inside hardware designs are distilled and represented by GNNs; the temporal knowledge (i.e., relative ordering of logic transformations) in synthesis flows can be imposed on hardware designs by combining a virtually added supernode or a sequence processing model with conventional GNN models. Evaluation on 3.3 million data points shows that the testing mean absolute percentage error (MAPE) on designs seen and unseen during training are no more than 1.2% and 3.1%, respectively, which are 7-15X lower than existing studies.

==> reviews.tex <==
============================================================================ 
DAC 2022 Reviews for Submission #1159
============================================================================ 

Title: Hybrid Graph Models for Logic Optimization via Spatio-Temporal Information
Authors: Nan Wu, You-Young Lee, Yuan Xie and Cong Hao


============================================================================
                            REVIEWER #1
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
           Clarity / Writing Style (1-5): 4
      Originality / Innovativeness (1-5): 3
    Impact of Ideas and/or Results (1-5): 4
            OVERALL RECOMMENDATION (1-5): 3

Summarize shortly the contributions of the paper in your own words.
---------------------------------------------------------------------------
The paper proposes a hybrid GNN targeted for logic synthesis. The hybrid approach captures spatio-temporal properties of netlists and flows to improve quality of results predictions and generalize to unseen designs. The results indicate that such an approach improves on current approaches and is closer to the ABC baseline.
---------------------------------------------------------------------------


Strengths
---------------------------------------------------------------------------
+ Paper is well written and concepts are explained
+ Adds flow information to the model
+ Proposes approach with high generalization without retraining
---------------------------------------------------------------------------


Weaknesses
---------------------------------------------------------------------------
- Non-standard netlist representation
- Design specific flows are not realistic
- Unclear what changes to models require retraining
- Comparison is against inferior models
---------------------------------------------------------------------------


Main Discussion of Paper
---------------------------------------------------------------------------
While adding flow information to the model can improves accuracy and generalize to unseen designs, it can not be considered as a breakthrough and thus the novelty of the approach is minimal. The techniques used such as the super node in GNN are not original to this work.

The authors capture the synthesis flow based on abc's transformations. However, the 7 captured transformations are macro steps in ABC. How would additional/micro transformations affect the accuracy of the predictions. Would the temporal model need to be retrained in that case and how feasible is that ?

This work represents the spatial properties of netlist by capturing the node types and operation types. In section 3.1, only 3 types of gates are mentioned. How would other types of gates influence the prediction and why didn't the authors use a standard representation such as AIG. This can help avoid re-training any time a new gate type is added.

Finally, the work compares against LSTM and CNN which are inferior in representing netlists. It would have been better if the authors compared against vanilla GNN implementation. 

While discussing the results of the evaluation of the different models in section 4.3, GNN-S is found to be inferior to GNN-H. The authors state earlier in the paper the 3 drawbacks of GNNS but they should should describe the major contributing reason, if any, behind the degradation. This can help advance further research in the field.
---------------------------------------------------------------------------


Most prominent Strength or Weakness
---------------------------------------------------------------------------
Comparison is against inferior models such as CNN.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #2
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
           Clarity / Writing Style (1-5): 4
      Originality / Innovativeness (1-5): 2
    Impact of Ideas and/or Results (1-5): 3
            OVERALL RECOMMENDATION (1-5): 3

Summarize shortly the contributions of the paper in your own words.
---------------------------------------------------------------------------
The paper present a method to estimate QoR in logic synthesis applications. The idea is to improve on existing methods by using simultaneously spatio-temporal information coming from hardware design and synthesis flow respectively. The method improves the mean absolute percentage error as compared to state-of-the-art.
---------------------------------------------------------------------------


Strengths
---------------------------------------------------------------------------
+ Interesting novel idea to use both spatial and temporal information from logic synthesis and design. 
+ Results compared on mapped design (7nm) compared to 2 previous works on same topic. 
+ Exhaustive description of the methods, figures, and setup.
---------------------------------------------------------------------------


Weaknesses
---------------------------------------------------------------------------
- Limited novelty on top of [17]
- Limited scalability of the method (no data on runtime)
- Evaluated on only 5 unseen designs during training
---------------------------------------------------------------------------


Main Discussion of Paper
---------------------------------------------------------------------------
- The novelty of the paper seems limited. Since LSTM were already employed in [17], the "only" difference seems the employment of the GNN. Nevertheless, I found the paper interesting and well written. The flow is well explained and Figure 3 is particularly helpful and illustrative. The motivation and novel contributions are clearly presented. 
- The experimental setup is complete and give exhaustive information. 

Few points: 
- The method is evaluated on few "unseen" designs (5). Why not all EPFL benchmarks are employed? Is this a scalability problem (for instance I noticed the hyp design is missing). Is this a limitation of the methods you compared to or is this a limitation of the presented method? Details in this direction should be added. 
- There are no data on scalability but a discussion paragraph. While generalization is thoroughly discussed (with seen and unseen designs), the runtime is instead completely disregarded. How is the runtime as compared to other similar works? It seems form the discussion that the method have scalability issues on large designs.
---------------------------------------------------------------------------


Most prominent Strength or Weakness
---------------------------------------------------------------------------
+ Interesting novel idea to use both spatial and temporal information from logic synthesis and design.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #3
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
           Clarity / Writing Style (1-5): 4
      Originality / Innovativeness (1-5): 3
    Impact of Ideas and/or Results (1-5): 3
            OVERALL RECOMMENDATION (1-5): 3

Summarize shortly the contributions of the paper in your own words.
---------------------------------------------------------------------------
The paper proposes some novel ML approaches for QoR estimations of logic synthesis flows, exploiting spatio-temporal information from hardware designs and logic synthesis flows in order to forecast performance of various synthesis flows on different designs.
---------------------------------------------------------------------------


Strengths
---------------------------------------------------------------------------
+ The paper is very well written and organized
+ The proposed techniques are well described and validated by a large set of experimental results
---------------------------------------------------------------------------


Weaknesses
---------------------------------------------------------------------------
- The preliminary part should be extended
- The dataset generation should better motivated
---------------------------------------------------------------------------


Main Discussion of Paper
---------------------------------------------------------------------------
Very interesting, well written paper. It contains a high degree of novelty. 

The ideas presented in the paper are easy to understand. The paper is very well structured and organized, and I think that it describes a very interesting result. 

The paper contains an extensive set of experimental results
.
The benchmarks described in the tables are few; the authors should show a bigger set of results. 

The authors should also discuss the computational time of the proposed methods.
---------------------------------------------------------------------------


Most prominent Strength or Weakness
---------------------------------------------------------------------------
The proposed techniques are well described and validated by a large set of experimental results.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #4
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
           Clarity / Writing Style (1-5): 5
      Originality / Innovativeness (1-5): 4
    Impact of Ideas and/or Results (1-5): 3
            OVERALL RECOMMENDATION (1-5): 3

Summarize shortly the contributions of the paper in your own words.
---------------------------------------------------------------------------
This paper proposes hybrid graph models with GNN and LSTM towards logic optimization utilizing spatio-temporal information. The proposed models enable to accurately estimate the PPA values of the practical benchmark circuits in comparison with baseline methods.
---------------------------------------------------------------------------


Strengths
---------------------------------------------------------------------------
+ The idea combining GNN with LSTM is interesting
+ The accuracy results look great
---------------------------------------------------------------------------


Weaknesses
---------------------------------------------------------------------------
- No comparison with commercial EDA tools
- The basic assumption is not realistic
- The computation overhead of the proposed method should be discussed
---------------------------------------------------------------------------


Main Discussion of Paper
---------------------------------------------------------------------------
1. The idea combining GNN with LSTM is interesting. The estimation accuracy looks very good in comparison with the baseline method. But the benefit derived from the proposed method should be more clearly written. For example, I guess users of commercial EDA tools (such as logic synthesis tools) just put "compile" command rather than the 100,000 flows in a single circuit design. Since "logic optimization" is included in the paper title, the logic optimization results by the proposed methods should be compared with the commercial EDA tools in order to further improve the advantage.

2.  The papers say that the accuracy can be further improved by increasing the layer of the GNN. If so, I think the computation overhead of the proposed method should be evaluated.

3. The problem formulation in Section 3.1 is not realistic. The actual circuits have not only AND/OR/NOT gates but also much more complex logic gates with multiple input pins. What happens if we employ logic gates such as NAND3?
---------------------------------------------------------------------------


Most prominent Strength or Weakness
---------------------------------------------------------------------------
- Performance comparison should be further analyzed
---------------------------------------------------------------------------

